From Cloud to Edge: A First Look at Public Edge Platforms

Public edge platforms have drawn increasing attention from both academia and industry. In this study, we perform a first-of-its-kind measurement study on a leading public edge platform that has been densely deployed in China. Based on this measurement, we quantitatively answer two critical yet unexplored questions. First, from end users' perspective, what is the performance of commodity edge platforms compared to cloud, in terms of the end-to-end network delay, throughput, and the application QoE. Second, from the edge service provider's perspective, how are the edge workloads different from cloud, in terms of their VM subscription, monetary cost, and resource usage. Our study quantitatively reveals the status quo of today's public edge platforms, and provides crucial insights towards developing and operating future edge services.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typset multiple affiliations (Christoph Sommer)

==> back.tex <==
\section{Background}

==> fig-cpu-var.tex <==
% !TeX root = main.tex
\begin{figure}[t]
	\centering				
	\begin{minipage}[b]{0.23\textwidth}
	\includegraphics[width=1\textwidth]{figs/cpu_balance_nc_new}
	\subcaption{Cross-server CPU usage}
	\label{fig:cpu-balance-nc}
	\end{minipage}	
	~		
	\begin{minipage}[b]{0.23\textwidth}
	\includegraphics[width=1\textwidth]{figs/cpu_balance_node_new}
	\subcaption{Cross-site CPU usage}
	\label{fig:cpu-balance-node}
	\end{minipage}
	
	\caption{\textbf{The CPU usage across servers/\nodes is highly unbalanced.}
		All \nodes are randomly sampled from Guangdong Province, and the servers are from a random \node.
		A server's CPU usage is calculated as the weighted (by requested cores) CPU usage of all its hosted VMs, and a \node's CPU usage is averaged across all its servers.
		For each figure: all numbers are normalized to the smallest one.}
	\label{fig:cpu-var}
\end{figure}

==> fig-hop-num.tex <==
% !TeX root = main.tex

\begin{figure}
	\centering					
	\includegraphics[width=0.4\textwidth]{figs/hop_num}
	\caption{\textbf{Hop numbers} from users to edge/cloud platforms.}
	\label{fig:hop-num}
\end{figure}

==> fig-sale.tex <==
% !TeX root = main.tex

\begin{figure}[t]
	\centering					
	\includegraphics[width=0.4\textwidth]{figs/sale}
	\caption{
		The fraction of CPU cores and memory sold out at the granularity of machines and \nodes.}
	\label{fig:sale}
\end{figure}

==> intro.tex <==
\section{Introduction}

We are witnessing a tremendous shift of data and computation being decentralized from cloud datacenters to network edges.
Favourably endowed with low delay and other advantages, edge computing has reached its eve with much momentum, along with other interdependent techniques like IoT, 5G, and AR/VR.
Different paradigms have been proposed to materialize edge computing, e.g., cloudlet~\cite{satyanarayanan2009case}, fog computing~\cite{bonomi2012fog}, and MEC~\cite{mec-whitepaper}.
Among those forms, we believe \textit{public edge platform} is more likely to achieve commercial success.
This is mainly because it inherits the key spirits from the cloud computing that has been dominating the IT discourse in the past decade.
Major cloud providers are building their public edge platforms.
In US, Amazon and Microsoft have released their edge solutions recently, i.e., AWS Local Zones~\cite{aws-local-zones} in Dec. 2019 and Azure Edge Zone~\cite{azure-edge-zone} in Mar. 2020.
Both of them provide multi-tenant edge resources near end users and companies.
Those platforms are still at very primitive stage and only available at a few cities such as LA and NYC.

\textbf{\sys}\footnote{Name anonymized for double-blind review.} (\textbf{n}ext-generation \textbf{e}dge \textbf{p}latform) is our solution to edge computing.
\sys is a multi-tenant edge platform that is launched since early 2018 and temporarily operates in China.
In June, \sys has incorporated about two orders of magnitudes larger number of datacenters (DC) than aforementioned edge providers and covered every province in China.
As a result, \sys has become a leading edge provider and serve a large number of commercial applications as well as millions of users.
With its early-stage success, we believe it's time to review the status quo through in-depth measurements and analysis, which may shed light on future edge research.

Based on \sys, this work seeks to answer two \textit{critical} yet \textit{unexplored} questions of public edge platforms:
(1) what's the edge performance (mostly network-wise) from the end-user perspective;
(2) what're the edge workloads from the edge developer and platform perspectives.
The first one demystifies how much improvements of experience an edge platform can bring to end users, and the second one reveals how traditional DC methodologies and techniques shall be transformed to fit into the edge workloads.
In a nutshell, looking into these two questions helps edge researchers and practitioners understand how far is edge computing from its prospects and what does it take to reach the tipping point of the edge ecosystem.

\textit{\textbf{Edge-cloud comparison}}
For both aspects to explore, we compare \sys to populr public cloud platforms, to demystify their differences and guide how the cloud DCs shall be transformed into edges.
We make the comparison fair and meaningful with best efforts:
since \sys is located in China, we use Alibaba Cloud Elastic Computing Service~\cite{ali-ecs} (\cloudsys for short), the leading cloud provider in China, as the first cloud-side reference.
We use \cloudsys for the comparison of performance ($\S$\ref{sec:performance}) and billing cost ($\S$\ref{sec:cost}).
However, \cloudsys (or other major Chinese cloud providers) do not publish their \textit{complete} workloads traces\footnote{We are aware of other public cloud workloads datasets from Chinese cloud providers~\cite{alibaba-cloud-data}. However, those datasets only come from a \textit{subset} VMs of the platform so not representative enough as we have analyzed.}.
To this end, we use the Azure traces (the 2019 version)~\cite{cortez2017resource} as the second cloud reference.
While the locations may affect the platform workloads, we believe the conclusions drawn in this study are faithful, considering the large quantity of investigated objects.

\textbf{Characterizing edge performance}
Edge computing brings hardware resources close to users, thus is supposed to deliver better user experience, especially at network-wise.
To demystify the performance of \sys, we tested the end-to-end network latency and typical edge applications on \sys.

\textit{(1) End-to-end network latency ($\S$\ref{sec:network-delay}).}
To understand how close \sys's services are to end users,
we performed a country-wise network delay measurement through crowdsourcing.
The study involves 158 end users across 41 cities in China and we run our customized testing tool on their mobile devices.
In total we received 385 testing results under various network conditions, i.e., WiFi/LTE/5G, where each testing obtains the round-trip time (RTT) to each DC deployed by \sys and \cloudsys.
The RTT is also broken down to per-hop latency.

\textit{(2) Application-level performance ($\S$\ref{sec:app-performance}).}
We built two typical applications that are commonly envisioned as the killer apps for edge computing: cloud gaming and live streaming.
We set up 1 edge server and 3 cloud servers at different locations, and used 4 different devices to test the application performance.
The testings are performed by the authors across different locations and network conditions.
We also built a semi-automatic toolkit that can extract and break down the end-to-end application quality-of-experience (QoE).

\textbf{Characterizing edge workloads}
Understanding what kinds of applications and workloads are running on edge platforms is important to both system providers and developers.
Thus, we collected 3-month usage traces of \textit{all} Infrastructure-as-a-Service (IaaS) VMs running on \sys, and compare it to a major cloud platform Azure~\cite{cortez2017resource}.
This work targets IaaS VMs, because they contribute to most of the subscriptions and traffic at the current stage of \sys.

\textit{(3) Characteristics of edge apps/VMs ($\S$\ref{sec:vm-type}).}
Who are the customers or what applications have been built atop \sys in practice, and what kinds of VM subscriptions they have made?
Looking into those basic questions, we can reveal the reality and hype of killer apps for edge computing, and demystify how an edge app or service is organized across VMs.

\textit{(4) Monetary cost of edge apps ($\S$\ref{sec:cost}).}
Besides many comparisons between cloud and edge, a missing piece from all prior literature is the billing method.
We examine the billing difference between \sys and \cloudsys, and point out the rationales behind.
Based on the collected traces, we further investigate whether and to what extend \sys can reduce the monetary cost for edge developers.
The comparison is made to a cloud-version of those apps simulated by the same traces.

\textit{(5) Resource usage and load balance ($\S$\ref{sec:vm-usage}, $\S$\ref{sec:resource-allocate}).}
Keeping hardware resources in healthy status is critical to multi-tenant platforms.
We first inspect the overall resource usage and its across-time variance from single-vm perspective.
We then dive into whether the resource usage is balanced across machines/\nodes and across the same app's VMs.
The former one verifies the VM placement strategy made by edge platform,
and the latter peeps into how edge developers schedule traffic (or requests) from end users to their geo-distributed VMs.

\textbf{Summarized findings}
Our measurements and analysis lead to several insightful observations as summarized below.

\textit{(i) Network latency --}
The current deployment of \sys offers lower network delay and smaller jitter compared to \cloudsys.
Based on the crowdsourcing results, the median RTTs between users and the nearest edge DC are 16.1ms/37.6ms/10.4ms for WiFi/LTE/5G networks, which are 1.47$\times$/1.33$\times$/1.23$\times$ faster than the nearest cloud DC.
The reduced network jitter is even more profound, i.e., around 5$\times$ smaller RTT coefficient of variation (stddev/mean).
However, such performance can not (or barely) meet the requirements of some delay-critical applications such as cloud VR/ (20ms/5ms)~\cite{cloud-vr} and autonomous driving (10ms)~\cite{v2x-whitepaper}.
The nearest edge is still 5--12 (median: 8) hops away from end users, instead of 1--2 hops as commonly envisioned for edge computing~\cite{mec-whitepaper,satyanarayanan2009case}.
Such performance can be further improved by a geographically denser deployment of DCs, and more importantly, sinking the DCs into the operator's core network.

\textit{(ii) Application performance --}
Placing gaming backend on nearby edges can noticeably improve the response delay compared to distant clouds and achieve less than 100ms response delay.
To further enhance the gaming experience, we need to improve the server-side gaming execution speed, e.g., through higher CPU parallelism or hardware acceleration, as network latency is no longer the major bottleneck.
For live streaming...
\Note{to update}

\textit{(iii) Edge apps and workloads are observably different from cloud}.
Edge services are deployed to a larger number of VMs (1.6$\times$ higher ratio with $\ge$50 VMs), and the VMs are often equipped with more hardware resources, including both CPU cores (median: 8 vs. 1) and memory (median: 32GBs vs. 4GBs).
However, the resource utilization of edge apps is much lower than cloud (6$\times$ for mean CPU usage), which indicates a common resource over-provision phenomenon.
Such difference amplifies existing challenges when migrating from clouds to edges, e.g., the bin-packing problem of fitting applications to physical machines~\cite{conf/asplos/DelimitrouK14,meisner2011powernap}.
We identify two possible reasons to the cloud-edge workloads difference:
edge apps are mostly delay-critical and the usage patterns from end users exhibit high temporal skewness, which forces developers to allocate more resources;
it remains difficult for developers to understand the resource demand at different locations before deployment so they tend to be conservative.
%and once deployed, the dynamic resource scaling for IaaS VMs incurs high overhead.

\textit{(iv) \sys can significantly save the monetary cost of the edge apps.}
Assuming the data coming from nearby users, \sys offers much cheaper network billing compared to cloud.
As a result, deploying edge apps on \sys can reduce the overall monetary cost by about 45\% on average, and up to 98\% for network billings alone.
Edge apps deployed on \sys are mostly network-intensive, and the bandwidth cost often constitute most of their billing cost.
In fact, saving money might be the most practical and attractive incentive for developers to move from cloud to edge.
Given that, two kinds of apps may not benefit in this aspect: (1) apps with high hardware resource demand but less network demand, as \sys charges slightly higher on hardware resources; (2) apps with very high network usage variance across time, as \sys only provides coarse-grained billing method due to its limited elasticity.

\textit{(v) The resource usage (load) is highly unbalanced across machines/\nodes and the same app's VMs.}
The CPU/bandwidth usage gap can be up to 14$\times$ across the machines from the same \node and 731$\times$ across \nodes from the same province.
For a half edge apps, their 95th-percentile VM load is 3$\times$ higher than their 5th-percentile VM load.
% TODO: revised
Such observations expose the imperfections about \sys's VM placement strategies and edge developers' traffic routing algorithms.
We identify several challenges to achieve load balance in public edge platforms, including the changing usage pattern of single VM, unawareness of the geo-sensitive resource demand before deployment, and the decoupled VM placement and end-user request scheduling strategies.

\textbf{Contributions}
To our knowledge, this work presents the first comprehensive measurement study on a commercial public edge platform, either from the performance or workloads aspects.
Our main contributions are summarized as follows.
(1) A country-wise network delay measurement and its breakdown from end devices to geo-distributed edge/cloud DCs, which reveals to what extend edge platform can improve the delay and what's the bottleneck to be further optimized.
(2) The implementation and profiling of two killer applications for edge computing, i.e., cloud gaming and live streaming, to explore whether edges can help deliver those envisioned prospects;
(3) A characterization of edge workloads through a complete VM usage trace, which demystifies its key difference from cloud workloads and identifies the imperfections and challenges in managing edge resources.
(4) An analysis of the monetary cost to deploy service on edge platform, which is highlighted as an ignored incentive to move from clouds to edges.


==> lessons.tex <==
\section{Experiences and Lessons Learned}

What are important in building edge computing platforms? Possible future directions.

Nodeless?

==> schedule.tex <==
\section{Edge Resource Scheduler}

\textbf{Intra-\node res schedule vs. inter-\node res schedule vs. request schedule}

\subsection{Motivating Dynamic Resource Scheduling}

\subsubsection{Requests Skewness Across Edges}

In the granularity of VMs, machines, \nodes.

Same user's VMs across different \nodes.

More skewed than cloud

\subsubsection{The potential improvement}

Show that the network cost of edge provider can be reduced even without reducing the total network usage due to two reasons. First, smooth the traffic usage by locating VMs with different temporal usage pattern; second, move VMs to \nodes where network price is cheaper.

Show that we can estimate the uppper bound of latency penalty by inter-edge rtt.

\subsection{Problem Formulation}

\noindent \textbf{Assumptions}
For now, we only schedule the resources (in the form of VMs) but not requests. When a VM is moved from one \node to another, the requests that used to route to that virtual machine will still be, but in a different \node.
The scheduling is mainly designed from the perspective of edge provider.

\noindent \textbf{Symbols and terms}:
$vm_{i\in\{1,2,...,k\}}$ are the virtual machines to be scheduled,
$nc_{i\in\{1,2,...,m\}}$ are the networked machines that can host the VMs,
and $nd_{i\in\{1,2,...,n\}}$ are the geo-distributed \nodes comprised of many machines.
An application $app_{i\in\{1,2,...,l\}}$ serves user requests through one or many $vm$s.
A placement $\varrho$, or a resource scheduling strategy, maps each virtual machine $vm_i$ to a networked machine $nc_{\varrho(i)}$.
We use $\mathcal{P}(nc_i)$ or $\mathcal{P}(nd_i)$ to represent the indexes of $vm$s that are hosted in the machine $nc_i$ or \node $nd_i$ under the current resource placement.
Our goal is to find an optimal $\varrho$ that makes balance among the system metrics concerned.
Next, we will look into the constraints and optimization goals of $\varrho$.

\noindent \textbf{Scheduling Goals}
(1) To reduce the network cost charged by the network operators.
(2) To balance the resource usage. Given the total computations, balancing the CPU usage is critical to service avaiability and relability.
Since we only schedule resource but not requests, we cannot further balance the resource usage inside a VM.
Thus, our target is to balance the overall resource usage (mainly for CPU) for each networked machine across time, and the average resource usage across machines.
(3) To reduce possible latency penalty caused by VM migration.

\noindent \textbf{Hardware constraint}
For each $nc$, the hardware constraint must be respected..

\begin{equation}
\begin{split}
& \sum_{j \in \mathcal{P}(nc_i)}{CPU(vm_j)} < CPU(nc_i), i=1,2,...,m \\
& \sum_{j \in \mathcal{P}(nc_i)}{MEM(vm_j)} < MEM(nc_i), i=1,2,...,m \\
\end{split}
\end{equation}

Here, $CPU(t)$/$MEM(t)$ is the number of CPU cores or memory size that needed by a virtual machine (when $t$ is a $vm$) or available on a networked machine (when $t$ is a $nc$).


\noindent \textbf{Modeling the network latency penalty}
As a $vm$ migrates from $nc_i$ in old resource placement to $nc_j$ in a new resource placement, we model the latency penalty by the round-trip time between those two machines $L_{i,j}$. The new placement should satisfy the user-specified latency requirement, i.e., it shall not exceed an tolerable latency increment.

\begin{equation}
{L_{\varrho_1(i),\varrho_2(i)}} \le \mathcal{L}_{app(i)}, i=1,2,...,m
\end{equation}

%\begin{equation}
%\text{LAT\_INC}=\frac
%{\sum_{i=1}^{k}{L_{\varrho_1(i),\varrho_2(i)}} \times T(vm_i)}
%{\sum_{i=1}^{k}{T(vm_i)}} \\
%\end{equation}

Here, we estimate the upper bound of latency increase when we switch from resource placement $\varrho_1$ to $\varrho_j$.
$\mathcal{L}_{j}$ is the tolerable latency increment of $app_j$, and $app(i)$ is the index of the application type of $vm_i$.


\noindent \textbf{Modeling the network cost}
As aforementioned, the operators charge the \sys provider based on the peak bandwidth per day for each \node.
We use $\vec{b}_i$ to denote the recorded traffic usage of $vm_i$ in a day (sampled every 5 minutes in our dataset, 288 samples per day). 

\begin{equation}
\begin{split}
& net\_cost(i) =\max{(\sum_{j \in \mathcal{P}(nd_i)}{\vec{b}_j})} \\
& \text{NET\_COST} =\sum_{i=1}^{n}{(net\_cost(i)*net\_price(i))} \\
\end{split}
\end{equation}

Here, the sum of $\vec{b}_i$ is element-wise, and the $net\_price(i)$ is the unit price of network bandwidth in $nd_i$, e.g., \$100/Mbps.
Note that $net\_price$ varies across different geo-locations and operators.


\noindent \textbf{Modeling the resource balance across time}
We use the coefficient of variation ($c_v$) to represent the temporal resource usage variance for each $nc$.

\begin{equation}
\begin{split}
& cpu\_var(i) =c_v(\sum_{j \in \mathcal{P}(nc_i)}{(\vec{c}_j \times CPU(vm_j))}) \\
& \text{VAR\_TIME} =\frac{1}{m}(\sum_{i=1}^{m}{cpu\_var(i)}) \\
\end{split}
\end{equation}

Here, $\vec{c}_i$ is the cpu usage of $vm_i$ in a day (sampled every 2 minutes in our dataset, 720 samples per day).


\noindent \textbf{Modeling the resource balance across machines}
We use the coefficient of variation
\begin{equation}
\begin{split}
& cpu_{avg}(i)=\frac
{\sum_{j \in \mathcal{P}{(nc_i)}}{avg(\vec{c_j}) \times CPU(vm_j)}}
{\sum_{j \in \mathcal{P}{(nc_i)}}{CPU(vm_j)}} \\
& \text{VAR\_NC} =v_c({cpu_{avg}(1), cpu_{avg}(2), ..., cpu_{avg}(m)}) \\
\end{split}
\end{equation}


\noindent \textbf{Optimization}
The goal is to collectively reduce NET\_COST, VAR\_TIME, VAR\_NC, while respecting the hardware constraint and applications' latency requirement.

\noindent \textbf{Explosive search space}
The potential search space (number of valid placement) is estimated to be XXX (too large).

\subsection{Optimizations}

1. First allocate vms to \nodes, optimizing for NET\_COST only. Then allocate vms to machines, optimizing for resource usage balance.

2. Cluster all \nodes into sub-areas, so that the optimal placement of each sub-area can be computable.

3. Using genetic algorithm?


%\input{schedule_algo}

==> schedule_algo.tex <==
% !TeX root = main.tex

%\vspace{-5pt}
\let\oldnl\nl% Store \nl in \oldnl
\newcommand{\nonl}{\renewcommand{\nl}{\let\nl\oldnl}}% Remove line number for one line
\begin{algorithm}
	
\footnotesize
\caption{Resource Scheduling}\label{algo:tagging}
\SetKwInOut{Input}{input}
\SetKwInOut{Output}{output}
\Input{
$vm_1$,$vm_2$,...,$vm_k$: virtual machines to be migrated \\
$nc_1,nc_2,...,nc_m$: networked machines that host VMs \\
$nd_i,nd_2,...,nd_n$: geo-distributed \nodes containing many $nc$s \\
$p(i)$: old placement that $vm_i$ is hosted on $nc_{p(i)}$\\
}
\Output{
$p'(i)$: new placement that $vm_i$ is hosted on $nc_{p'(i)}$\\
}




xxx\\
xxx\\
xxx\\

$Q$ $\gets$ initialize upload queue\\
%$groups$ $\gets$ divide the query time range into groups based on $window\_size$\\
$groups$ $\gets$ divide the query time range into groups \\
\For(\tcp*[h]{rapid attempting}){$g$ in $groups$}{
	\lIf{any frame in $g$ is $P$/$N$}{
		pass
	}
	\lElseIf{any frame in $g$ is $U$}{
		add frame to $Q$
	}
	\uElse{
		$f$ $\gets$ pick a random frame from $g$\\
		process and tag $f$ with $op$\\
		\lIf{$f$ tagged as $U$}{
			add $f$ to $Q$
		}
	}
}
\While(\tcp*[h]{work stealing}){$Q$ is not empty}{
	$f \gets Q$.tail(); $g$ $\gets$ enclosing group of $f$ \\
	$f1$ $\gets$ an untagged frame within $g$ \\
	process and tag $f1$ with $op$ \\
	\lIf{$f1$ tagged as $P$/$N$}{
		remove $f$ from $Q$
	}
}
%\notettx{use even smaller fonts? like footnotesize}
\end{algorithm}
%\vspace{-10pt}

==> tab-app-type.tex <==
\begin{table}[t]
\scriptsize
\begin{tabular}{|l|l|l|l|l|l|}
\hline
 & \# of VMs & downlink/uplink & CPU cores & Memory & Storage \\ \hline
T1 &  &  &  &  &  \\ \hline
T2 &  &  &  &  &  \\ \hline
T3 &  &  &  &  &  \\ \hline
\end{tabular}
\caption{Classification of top 50 edge apps on \sys.}
\label{tab:app-classification}
\end{table}

==> tab-compare.tex <==
\begin{table}[!t]
\footnotesize
\begin{tabular}{l|L{3cm}|L{4cm}|}
 & \textbf{\# of \nodes in China} & \textbf{hw resources per \node}  \\ \hline
\textbf{\cloudsys} & 10, unchanged since 201X & Almost unlimited, high scalability and elasticity.  \\ \hline
\textbf{\sys} & 169 (expected to grow to >1000 at the end of 2020) & Typically tens of machines, highly constrained by the environmental infrastructure, e.g., space and electricity.  \\ \hline
\end{tabular}
\caption{A high-level comparison of \sys and \cloudsys.}
\end{table}

==> tab-rtt-range.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}RTT\\ bound (ms)\end{tabular}} & \multicolumn{3}{c|}{\textbf{WiFi}} & \multicolumn{3}{c|}{\textbf{LTE}} & \multicolumn{3}{c|}{\textbf{5G}} \\ \cline{2-10} 
 & 10 & 20 & 30 & 10 & 20 & 30 & 10 & 20 & 30 \\ \hline
\textbf{Edge} & 1.4 & 8.9 & 28.9 & 0.0 & 0.2 & 2.0 & 1.4 & 15.0 & 34.7  \\ \hline
\textbf{Cloud} & 0.1 & 0.5 & 1.5 & 0.0 & 0.0 & 0.1 & 0.0 & 1.4 & 3.1 \\ \hline
\end{tabular}
\caption{\textbf{The number of edge/cloud \nodes available for end users within certain RTT bound on average.} \mwx{May move to appendix}}
\label{tab:rtt-range}
\vspace{-10pt}
\end{table}
